Indexing Finite-State Automata Using Forward-Stable Partitions

An index on a finite-state automaton is a data structure able to locate specific patterns on the automaton's paths and consequently on the regular language accepted by the automaton itself. Cotumaccio and Prezza [SODA '21], introduced a data structure able to solve pattern matching queries on automata, generalizing the famous FM-index for strings of Ferragina and Manzini [FOCS '00]. The efficiency of their index depends on the width of a particular partial order of the automaton's states, the smaller the width of the partial order, the faster is the index. However, computing the partial order of minimal width is NP-hard. This problem was mitigated by Cotumaccio [DCC '22], who relaxed the conditions on the partial order, allowing it to be a partial preorder. This relaxation yields the existence of a unique partial preorder of minimal width that can be computed in polynomial time. In the paper at hand, we present a new class of partial preorders and show that they have the following useful properties: (i) they can be computed in polynomial time, (ii) their width is never larger than the width of Cotumaccio's preorders, and (iii) there exist infinite classes of automata on which the width of Cotumaccio's pre-order is linearly larger than the width of our preorder.

==> Chapters/chapter5conclusions.tex <==

\section{Conclusions}\label{sec:conc}


In conclusion, in this paper we have presented all the orders proposed for building indices on NFAs using a BWT-based strategy. We have then introduced the concept of \textit{coarsest forward-stable co-lex order} (CFS order) of an NFA, which is a specific partial preorder over an NFA’s set of states. We have also proved its existence and uniqueness for each NFA. After that, we have compared the CFS order with the other types of orders that $(i)$ can be used for indexing an NFA using a BWT-based strategy, and that $(ii)$ always exist for any NFA. These are the co-lex orders and the maximum co-lex relation ~\cite{cotumaccio2021indexing,cotumaccio2022graphs}. Notably, in Theorem~\ref{main:th:1} we have demonstrated that the width of the CFS order is never larger than the width of these other orders. Furthermore, in Theorem~\ref{main:th:2} we have shown that there exist NFAs for which the width of the forward-stable co-lex order is $O(1)$, while the width of any co-lex order or the maximum co-lex relation is $O(\lvert Q \rvert)$, where $Q$ is the set of states of the NFA. Finally, Corollary~\ref{unique:cor} proved that the forward-stable co-lex order of any NFA can be computed in polynomial time.



